A Reinforcement Learning Environment for Directed Quantum Circuit Synthesis

With recent advancements in quantum computing technology, optimizing quantum circuits and ensuring reliable quantum state preparation have become increasingly vital. Traditional methods often demand extensive expertise and manual calculations, posing challenges as quantum circuits grow in qubit- and gate-count. Therefore, harnessing machine learning techniques to handle the growing variety of gate-to-qubit combinations is a promising approach. In this work, we introduce a comprehensive reinforcement learning environment for quantum circuit synthesis, where circuits are constructed utilizing gates from the the Clifford+T gate set to prepare specific target states. Our experiments focus on exploring the relationship between the depth of synthesized quantum circuits and the circuit depths used for target initialization, as well as qubit count. We organize the environment configurations into multiple evaluation levels and include a range of well-known quantum states for benchmarking purposes. We also lay baselines for evaluating the environment using Proximal Policy Optimization. By applying the trained agents to benchmark tests, we demonstrated their ability to reliably design minimal quantum circuits for a selection of 2-qubit Bell states.

==> content/2_preliminaries.tex <==
\section{BACKGROUND} \label{sec:preliminaries}

Due to the fact that this research is directed towards the subjects of quantum computing and reinforcement learning, the following section gives a short introduction to both fields and motivates the approaches to our following experiments. 
%Apart from conveying basic concepts, additional information about topics necessary for understanding the content of the following experiments is given.  

\subsection{Quantum Computing}
Quantum computing is an emerging technology distinguishing itself from classical computing fundamentally. A main difference is given by the usage of so-called quantum bits or qubits instead of classical bits as units of information storage.

\subsubsection{Qubits as Quantum states}
Qubits among other aspects differ from their classical counterparts by showing a characteristic named superposition. Superposition describes the ability of qubits to not only be in one of the discrete states 0 or 1, like a classical bit, but to be in any linear combination of 0 and 1 enlarging the available state-space from discrete to continuous. \cref{eq: qubitstate} defines the quantum state of one qubit in the Bra-Ket and vector-notation.

\begin{align}
    \ket{q} = \alpha \ket{0} + \beta \ket{1} = \begin{pmatrix}
        \alpha \\
        \beta
    \end{pmatrix}\; \; \; \; \; \;\alpha, \beta \; \in \;\mathbb{C}\label{eq: qubitstate}
\end{align}
%Since quantum computation commonly relies on the calculation with physical quantum particles, obeying the wave-particle dualism, the involved particles can be interpreted as waves. The coefficients $\alpha$ and $\beta$ represent the amplitudes of the respective wave-function of the wave $\ket{0}$ or $\ket{1}$. The probability of finding $\ket{q}$ in on of the substates $\ket{0}$ or $\ket{1}$ is then given by the squared amplitudes $|\alpha|^2$ or $|\beta|^2$ respectively. The characteristic of conventional random experiments that the probabilities of all possible outcomes add up to 1, is equivalent to the normalization of the state $\ket{q}$, $1 = \bra{q}\ket{q} = |\alpha|^2 + |\beta|^2$, and forms the only constraint on the linear combination of $\ket{0}$ or $\ket{1}$.\indent
Another aspect distinguishing qubits from classical bits is a characteristic called entanglement. Entanglement describes the possibility of correlating the states of multiple qubits, enabling the setup of complex relations between them. However, the simulation of such correlation using classical qubits is highly resource intensive, scaling exponentially with the number of involved qubits.  \indent 
Apart from the vector notation given in \cref{eq: qubitstate}, another option for the description of quantum states exists, which is called the density matrix representation given in \cref{eq: qubitmatrix}. 

\begin{align}
    \rho = \ket{q}\bra{q} = \begin{pmatrix}
        |\alpha|^2 & \alpha\beta^{*}\\
        \alpha^{*}\beta & |\beta|^2
    \end{pmatrix}\; \; \; \; \; \;\alpha, \beta \; \in \;\mathbb{C}\label{eq: qubitmatrix}
\end{align}
However, the usage of the density matrix formalism enables the depiction of states not decomposable into a set of vectors anymore. Such matrices correspond to a statistical ensemble of different quantum states also referred to as 'mixed states', while the states representable by simple vector notation are called 'pure states'. To compare two density matrices and hence two quantum states $\rho$ and $\widetilde{\rho}$, the fidelity $F$ as given in \cref{eq: fidelity} is used as a measure.

\begin{align}
    F(\rho,\widetilde{\rho}) = \biggl(tr\biggl(\sqrt{\sqrt{\rho}\widetilde{\rho}\sqrt{\rho}}\biggr)\biggr)^{2} \label{eq: fidelity}
\end{align}
When solely pure states are involved this equation simplifies to the expression given in \cref{eq: purefidelity}, while $\widetilde{q}$ is the vector representation of $\widetilde{\rho}$~\cite{Jozsa1994}.

\begin{align}
    F(\rho,\widetilde{\rho}) = |\bra{q}\ket{\widetilde{q}}|^2 \label{eq: purefidelity}
\end{align}
 In this work, we only consider pure quantum states in their vector representation and thus only the fidelity given in \cref{eq: purefidelity}. 

\subsubsection{Quantum-circuits}
With the qubit as the basic information storage unit in mind, the next important part of a computational process involves the available mathematical operations applicable to the present information. Quantum computers, similar to classical ones, rely on sets of logic gates as building blocks for all executable operations. Several of these so-called quantum logic gate sets exist. The quantum logic gates, or short quantum gates, included in these sets are implemented as quantum mechanical operators, represented by unitary matrices. When applied on a quantum state $\ket{\Phi}$ a quantum mechanical operator $U$ transforms the current state into a new one $\ket{\Phi'}$ according to \cref{eq: quantumtrafo}.

\begin{align}
    \ket{\Phi'} = U \ket{\Phi} \label{eq: quantumtrafo}
\end{align}
The unitarity aspect of the gates makes all operations relying on these gates unitary and hence reversible. (see \cref{subsec: quantumstateprep} for a proof) A generic unitary matrix working as a quantum mechanical operator on a single qubit can be defined according to \cref{eq: genericunitary}.

\begin{align}
    U = e^{i\frac{\gamma}{2}}\begin{pmatrix}
        \cos{\theta} e^{i\rho}\; \;\;\;\;\;\;\;\;\sin{\theta} e^{i\phi} \;\\
        \;-\sin{\theta} e^{-i\phi} \;\;\;\; \cos{\theta} e^{-i\rho}\;
        \end{pmatrix} \label{eq: genericunitary} 
\end{align}  
Out of this generic matrix, different quantum gates can be created by selecting specific values for the involved parameters. Furthermore, by leaving some of the involved parameters undefined the design of parameterized quantum gates is possible. %Classical examples of non-parameterized quantum gates are the Hadamard or the identity gate, whereas the rotation gates $R_{x}(\phi)$, $R_{y}(\phi)$ and $R_{z}(\phi)$ represent common parameterized gates. 
Another characteristic distinguishing quantum gates is their multiplicity, corresponding to the number of qubits the respective quantum gate acts upon. All above-mentioned gates including the general unitary given in \cref{eq: genericunitary} are single qubit gates. Examples of multiple qubits gates would be the CNOT acting on two qubits or the Toffoli gate acting on three qubits at once. \indent
An important characteristic of a quantum gate set is its strict universality, %given explicitly in the following definition. 
%\begin{definition}
    %Definition of Strict Universality: \\ A set of quantum gates S is said to be strictly universal if there exists a constant n0 such that for any n $\geq$ n0, the subgroup generated by S is dense in SU(2n), the group of unitary matrices with determinant 1 operating on n qubits~\cite{Aharonov2003}.
%\end{definition}

%Hence strict universality 
which describes the ability of a set to reproduce every possible transformation matrix with a finite combination of gates out of the respective set.
%Examples of universal quantum logic gate sets are the Clifford+T set and the Toffoli+H gate set. Since 
The Clifford+T is the gate set used in this study its included gates are given in their matrix representation in \cref{table : gatesets}~\cite{Aharonov2003,Kliuchnikov2013}.
\begin{table}[htbp]
\begin{center}
\adjustbox{max width=\linewidth}{
    \begin{tabular}{ |c|c|c| } 
        \hline
         Symbol (Name) & Matrix representation & Circuit notation\\ 
        \hline\hline
        \rule{0pt}{25pt} I (Identity)  &  $ \begin{pmatrix} 1 & 0 \\ 0 & 1 \\ \end{pmatrix} $ & \begin{quantikz}[thin lines]&\gate{I}&\end{quantikz}\\[15pt]
        \hline
        \rule{0pt}{25pt}H (Hadamard)  &  $ \frac{1}{\sqrt{2}}\begin{pmatrix} 1 & 1 \\ 1 & -1 \\ \end{pmatrix} $ & \begin{quantikz}[thin lines]&\gate{H}&\end{quantikz}\\[15pt]
        \hline
        \rule{0pt}{25pt}S   &  $ \begin{pmatrix} 1 & 0 \\ 0 & e^{i \frac{\pi}{2}} \\ \end{pmatrix} $ & \begin{quantikz}[thin lines]&\gate{S}&\end{quantikz}\\[15pt]
         \hline
        \rule{0pt}{40pt}CNOT   &  $ \begin{pmatrix} 1 & 0 & 0 & 0\\ 0 & 1 & 0 & 0\\0 & 0 & 0 & 1\\0 & 0 & 1 & 0\\ \end{pmatrix} $& \begin{quantikz}[thin lines]&\ctrl{1}&\\&\targ{}&\end{quantikz}\\[30pt]
         \hline
        \rule{0pt}{25pt}T   &  $ \begin{pmatrix} 1 & 0 \\ 0 & e^{i \frac{\pi}{4}} \\ \end{pmatrix} $ & \begin{quantikz}[thin lines]&\gate{T}&\end{quantikz}\\[15pt]
         \hline
    \end{tabular}
    }
    \caption{Table showing the gates included in the Clifford+T gate set together with their matrix representation and their circuit notation. The case shown for the CNOT-gate corresponds to the first qubit being the control bit.}
    \label{table : gatesets}
\end{center}
\end{table}

On the bottom line, a quantum circuit is a sequence of quantum gates acting upon a number of qubits. Hence the circuit can be seen as one big transformation matrix, transforming the incoming quantum state provided by the input qubits into an altered quantum state obtained on the output qubits. 
